Deep neural network surrogates for non-smooth quantities of interest in shape uncertainty quantification

We consider the point evaluation of the solution to interface problems with geometric uncertainties, where the uncertainty in the obstacle is described by a high-dimensional parameter $\boldsymbol{y}\in[-1,1]^d$, $d\in\mathbb{N}$. We focus in particular on an elliptic interface problem and a Helmholtz transmission problem. Point values of the solution in the physical domain depend in general non-smoothly on the high-dimensional parameter, posing a challenge when one is interested in building surrogates. Indeed, high-order methods show poor convergence rates, while methods which are able to track discontinuities usually suffer from the so-called curse of dimensionality. For this reason, in this work we propose to build surrogates for point evaluation using deep neural networks. We provide a theoretical justification for why we expect neural networks to provide good surrogates. Furthermore, we present extensive numerical experiments showing their good performance in practice. We observe in particular that neural networks do not suffer from the curse of dimensionality, and we study the dependence of the error on the number of point evaluations (that is, the number of discontinuities in the parameter space), as well as on several modeling parameters, such as the contrast between the two materials and, for the Helmholtz transmission problem, the wavenumber.

==> arxiv submission/slidesymbols.tex <==
% ======================================================================
% MACROS
% ======================================================================

% Operators

\providecommand{\Bdsymb}{\Gamma}                   % Tag for boundary operators
\providecommand{\Div}{\operatorname{div}}          % Divergence
\providecommand{\bDiv}{{\Div}_{\Bdsymb}}           % Surface divergence
\providecommand{\mDiv}{\operatorname{\sf div}}     % matrix divergence
\providecommand{\curl}{\operatorname{{\bf curl}}}  % Standard curl operator
\providecommand{\plcurl}{\operatorname{{\bf curl}}_{2D}} % Vectorial curl operator in 2D
\providecommand{\bcurl}{{\curl}_{\Bdsymb}}         % vectorial curl on the surface
\providecommand{\bscurl}{\operatorname{curl}_{\Bdsymb}} % scalar curl on a surface
\providecommand{\scurl}{\operatorname{curl}_{2D}}       % scalar curl in 2D
\providecommand{\mcurl}{\operatorname{{\bf\sf curl}}}   % matrix curl operator
\providecommand{\grad}{\operatorname{{\bf grad}}}       % standard gradient
\providecommand{\bgrad}{\grad_{\Bdsymb}}                % Surface gradient
\providecommand{\mgrad}{\operatorname{{\bf\sf grad}}}   % Matrix gradient for row vectors

\providecommand{\Dim}{\operatorname{dim}}            % dimension
\providecommand{\dim}{\Dim}
\providecommand{\Card}{\sharp}                       % numel of a set (cardinality)
\providecommand{\Vol}{\operatorname{Vol}}   % volume
\providecommand{\vol}{\Vol}
\providecommand*{\Meas}[2][]{\operatorname{meas}_{#1}({#2})} % measure
\providecommand*{\meas}[2][]{\Meas{#1}{#2}}
\providecommand*{\dist}[2]{\operatorname{dist}({#1};{#2})}   % distance
\providecommand*{\Dist}[2]{\dist{#1}{#2}}
\providecommand{\Det}{\operatorname{det}}                    % determinant
\providecommand{\Sgn}{\operatorname{sgn}}                    % sign
\providecommand*{\Kern}[1]{{\rm Ker}({#1})}                  % Kernel
\providecommand*{\Dom}[1]{{\rm Dom}({#1})}                   % Domain
\providecommand*{\Span}[1]{\operatorname{Span}\left\{{#1}\right\}}     % Span
\providecommand*{\Convex}[1]{\operatorname{convex}\left\{{#1}\right\}} % convex hull
\providecommand{\Supp}{\operatorname{supp}}                            % support
\providecommand{\supp}{\Supp}
\providecommand*{\Image}[1]{\mathrm{Im}({#1})}                         % Image
\providecommand*{\Range}[1]{\operatorname{Range}({#1})}                % Range
\providecommand{\rank}{\operatorname{rank}}                        % rank
\providecommand{\Rank}{\rank}
\renewcommand{\Re}{\operatorname{Re}}             % real part
\renewcommand{\Im}{\operatorname{Im}}             % imaginary part
\providecommand{\argmin}{\operatorname*{argmin}}  % argument yielding inf
\providecommand{\argmax}{\operatorname*{argmax}}  % argument yielding max
\providecommand{\nnz}{\operatorname{nnz}}         % no of nonzeros
\providecommand{\Id}{\Op{Id}}                     % Identity operator
\providecommand{\diam}{\operatorname{diam}}
\providecommand{\diag}{\operatorname{diag}}
\providecommand{\esssup}{\operatorname*{esssup}}
\providecommand{\essinf}{\operatorname*{essinf}}
\providecommand{\limsup}{\operatorname*{limsup}}

% Bold small letters (for vectors)

\newcommand{\Va}{{\mathbf{a}}}
\newcommand{\Vb}{{\mathbf{b}}}
\newcommand{\Vc}{{\mathbf{c}}}
\newcommand{\Vd}{{\mathbf{d}}}
\newcommand{\Ve}{{\mathbf{e}}}
\newcommand{\Vf}{{\mathbf{f}}}
\newcommand{\Vg}{{\mathbf{g}}}
\newcommand{\Vh}{{\mathbf{h}}}
\newcommand{\Vi}{{\mathbf{i}}}
\newcommand{\Vj}{{\mathbf{j}}}
\newcommand{\Vk}{{\mathbf{k}}}
\newcommand{\Vl}{{\mathbf{l}}}
\newcommand{\Vm}{{\mathbf{m}}}
\newcommand{\Vn}{{\mathbf{n}}}
\newcommand{\Vo}{{\mathbf{o}}}
\newcommand{\Vp}{{\mathbf{p}}}
\newcommand{\Vq}{{\mathbf{q}}}
\newcommand{\Vr}{{\mathbf{r}}}
\newcommand{\Vs}{{\mathbf{s}}}
\newcommand{\Vt}{{\mathbf{t}}}
\newcommand{\Vu}{{\mathbf{u}}}
\newcommand{\Vv}{{\mathbf{v}}}
\newcommand{\Vw}{{\mathbf{w}}}
\newcommand{\Vx}{{\mathbf{x}}}
\newcommand{\Vy}{{\mathbf{y}}}
\newcommand{\Vz}{{\mathbf{z}}}

% Small bold math characters

\providecommand{\Ba}{{\boldsymbol{a}}}
\providecommand{\Bb}{{\boldsymbol{b}}}
\providecommand{\Bc}{{\boldsymbol{c}}}
\providecommand{\Bd}{{\boldsymbol{d}}}
\providecommand{\Be}{{\boldsymbol{e}}}
\providecommand{\Bf}{{\boldsymbol{f}}}
\providecommand{\Bg}{{\boldsymbol{g}}}
\providecommand{\Bh}{{\boldsymbol{h}}}
\providecommand{\Bi}{{\boldsymbol{i}}}
\providecommand{\Bj}{{\boldsymbol{j}}}
\providecommand{\Bk}{{\boldsymbol{k}}}
\providecommand{\Bl}{{\boldsymbol{l}}}
\providecommand{\Bm}{{\boldsymbol{m}}}
\providecommand{\Bn}{{\boldsymbol{n}}}
\providecommand{\Bo}{{\boldsymbol{o}}}
\providecommand{\Bp}{{\boldsymbol{p}}}
\providecommand{\Bq}{{\boldsymbol{q}}}
\providecommand{\Br}{{\boldsymbol{r}}}
\providecommand{\Bs}{{\boldsymbol{s}}}
\providecommand{\Bt}{{\boldsymbol{t}}}
\providecommand{\Bu}{{\boldsymbol{u}}}
\providecommand{\Bv}{{\boldsymbol{v}}}
\providecommand{\Bw}{{\boldsymbol{w}}}
\providecommand{\Bx}{{\boldsymbol{x}}}
\providecommand{\By}{{\boldsymbol{y}}}
\providecommand{\Bz}{{\boldsymbol{z}}}

% Capital bold Characters

\newcommand{\VA}{{\mathbf{A}}}
\newcommand{\VB}{{\mathbf{B}}}
\newcommand{\VC}{{\mathbf{C}}}
\newcommand{\VD}{{\mathbf{D}}}
\newcommand{\VE}{{\mathbf{E}}}
\newcommand{\VF}{{\mathbf{F}}}
\newcommand{\VG}{{\mathbf{G}}}
\newcommand{\VH}{{\mathbf{H}}}
\newcommand{\VI}{{\mathbf{I}}}
\newcommand{\VJ}{{\mathbf{J}}}
\newcommand{\VK}{{\mathbf{K}}}
\newcommand{\VL}{{\mathbf{L}}}
\newcommand{\VM}{{\mathbf{M}}}
\newcommand{\VN}{{\mathbf{N}}}
\newcommand{\VO}{{\mathbf{O}}}
\newcommand{\VP}{{\mathbf{P}}}
\newcommand{\VQ}{{\mathbf{Q}}}
\newcommand{\VR}{{\mathbf{R}}}
\newcommand{\VS}{{\mathbf{S}}}
\newcommand{\VT}{{\mathbf{T}}}
\newcommand{\VU}{{\mathbf{U}}}
\newcommand{\VV}{{\mathbf{V}}}
\newcommand{\VW}{{\mathbf{W}}}
\newcommand{\VX}{{\mathbf{X}}}
\newcommand{\VY}{{\mathbf{Y}}}
\newcommand{\VZ}{{\mathbf{Z}}}

% Capital bold characters in math mode

\providecommand{\BA}{{\boldsymbol{A}}}
\providecommand{\BB}{{\boldsymbol{B}}}
\providecommand{\BC}{{\boldsymbol{C}}}
\providecommand{\BD}{{\boldsymbol{D}}}
\providecommand{\BE}{{\boldsymbol{E}}}
\providecommand{\BF}{{\boldsymbol{F}}}
\providecommand{\BG}{{\boldsymbol{G}}}
\providecommand{\BH}{{\boldsymbol{H}}}
\providecommand{\BI}{{\boldsymbol{I}}}
\providecommand{\BJ}{{\boldsymbol{J}}}
\providecommand{\BK}{{\boldsymbol{K}}}
\providecommand{\BL}{{\boldsymbol{L}}}
\providecommand{\BM}{{\boldsymbol{M}}}
\providecommand{\BN}{{\boldsymbol{N}}}
\providecommand{\BO}{{\boldsymbol{O}}}
\providecommand{\BP}{{\boldsymbol{P}}}
\providecommand{\BQ}{{\boldsymbol{Q}}}
\providecommand{\BR}{{\boldsymbol{R}}}
\providecommand{\BS}{{\boldsymbol{S}}}
\providecommand{\BT}{{\boldsymbol{T}}}
\providecommand{\BU}{{\boldsymbol{U}}}
\providecommand{\BV}{{\boldsymbol{V}}}
\providecommand{\BW}{{\boldsymbol{W}}}
\providecommand{\BX}{{\boldsymbol{X}}}
\providecommand{\BY}{{\boldsymbol{Y}}}
\providecommand{\BZ}{{\boldsymbol{Z}}}

\newcommand{\nablabf}{\boldsymbol{\nabla}}
\newcommand{\alphabf}{\boldsymbol{\alpha}}
\newcommand{\betabf}{\boldsymbol{\beta}}
\newcommand{\gammabf}{\boldsymbol{\gamma}}
\newcommand{\deltabf}{\boldsymbol{\delta}}
\newcommand{\epsilonbf}{\boldsymbol{\epsilon}}
\newcommand{\varepsilonbf}{\boldsymbol{\varepsilon}}
\newcommand{\zetabf}{\boldsymbol{\zeta}}
\newcommand{\etabf}{\boldsymbol{\eta}}
\newcommand{\thetabf}{\boldsymbol{\theta}}
\newcommand{\varthetabf}{\boldsymbol{\vartheta}}
\newcommand{\iotabf}{\boldsymbol{\iota}}
\newcommand{\kappabf}{\boldsymbol{\kappa}}
\newcommand{\lambdabf}{\boldsymbol{\lambda}}
\newcommand{\mubf}{\boldsymbol{\mu}}
\newcommand{\nubf}{\boldsymbol{\nu}}
\newcommand{\xibf}{\boldsymbol{\xi}}
\newcommand{\pibf}{\boldsymbol{\pi}}
\newcommand{\varpibf}{\boldsymbol{\varpi}}
\newcommand{\rhobf}{\boldsymbol{\rho}}
\newcommand{\varrhobf}{\boldsymbol{\varrho}}
\newcommand{\sigmabf}{\boldsymbol{\sigma}}
\newcommand{\varsigmabf}{\boldsymbol{\varsigma}}
\newcommand{\taubf}{\boldsymbol{\tau}}
\newcommand{\upsilonbf}{\boldsymbol{\upsilon}}
\newcommand{\phibf}{\boldsymbol{\phi}}
\newcommand{\varphibf}{\boldsymbol{\varphi}}
\newcommand{\chibf}{\boldsymbol{\chi}}
\newcommand{\psibf}{\boldsymbol{\psi}}
\newcommand{\omegabf}{\boldsymbol{\omega}}
\newcommand{\Gammabf}{\boldsymbol{\Gamma}}
\newcommand{\Deltabf}{\boldsymbol{\Delta}}
\newcommand{\Thetabf}{\boldsymbol{\Theta}}
\newcommand{\Lambdabf}{\boldsymbol{\Lambda}}
\newcommand{\Xibf}{\boldsymbol{\Xi}}
\newcommand{\Pibf}{\boldsymbol{\Pi}}
\newcommand{\Psibf}{\boldsymbol{\Psi}}
\newcommand{\Sigmabf}{\boldsymbol{\Sigma}}
\newcommand{\Upsilonbf}{\boldsymbol{\Upsilon}}
\newcommand{\Phibf}{\boldsymbol{\Phi}}
\newcommand{\Omegabf}{\boldsymbol{\Omega}}

% bold greek characters (math style)
% Comment axelo: \alphabf,... is inconsistent \with \Ba!
%                \Valpha,... and \Balpha added below
%                Also, for capital Greek letters \mathbf and \boldsymbol is the same!

% Bold upright capital greek letters for _V_ectors and Matrices
\newcommand{\VGamma}  {\mathbf{\Gamma}}
\newcommand{\VDelta}  {\mathbf{\Delta}}
\newcommand{\VTheta}  {\mathbf{\Theta}}
\newcommand{\VLambda} {\mathbf{\Lambda}}
\newcommand{\VXi}     {\mathbf{\Xi}}
\newcommand{\VPi}     {\mathbf{\Pi}}
\newcommand{\VPsi}    {\mathbf{\Psi}}
\newcommand{\VSigma}  {\mathbf{\Sigma}}
\newcommand{\VUpsilon}{\mathbf{\Upsilon}}
\newcommand{\VPhi}    {\mathbf{\Phi}}
\newcommand{\VOmega}  {\mathbf{\Omega}}

% _B_old italicized capital greek letters
\newcommand{\BGamma}  {\boldsymbol{\mathit{\Gamma}}}
\newcommand{\BDelta}  {\boldsymbol{\mathit{\Delta}}}
\newcommand{\BTheta}  {\boldsymbol{\mathit{\Theta}}}
\newcommand{\BLambda} {\boldsymbol{\mathit{\Lambda}}}
\newcommand{\BXi}     {\boldsymbol{\mathit{\Xi}}}
\newcommand{\BPi}     {\boldsymbol{\mathit{\Pi}}}
\newcommand{\BPsi}    {\boldsymbol{\mathit{\Psi}}}
\newcommand{\BSigma}  {\boldsymbol{\mathit{\Sigma}}}
\newcommand{\BUpsilon}{\boldsymbol{\mathit{\Upsilon}}}
\newcommand{\BPhi}    {\boldsymbol{\mathit{\Phi}}}
\newcommand{\BOmega}  {\boldsymbol{\mathit{\Omega}}}

% Bold upright lower case greek letters for _V_ectors and matrices (requires package upgreek)
\newcommand{\Valpha}     {\boldsymbol{\upalpha}}
\newcommand{\Vbeta}      {\boldsymbol{\upbeta}}
\newcommand{\Vgamma}     {\boldsymbol{\upgamma}}
\newcommand{\Vdelta}     {\boldsymbol{\updelta}}
\newcommand{\Vepsilon}   {\boldsymbol{\upepsilon}}
\newcommand{\Vvarepsilon}{\boldsymbol{\upvarepsilon}}
\newcommand{\Vzeta}      {\boldsymbol{\upzeta}}
\newcommand{\Veta}       {\boldsymbol{\upeta}} %
\newcommand{\Vtheta}     {\boldsymbol{\uptheta}}
\newcommand{\Vvartheta}  {\boldsymbol{\upvartheta}}
\newcommand{\Viota}      {\boldsymbol{\upiota}}
\newcommand{\Vkappa}     {\boldsymbol{\upkappa}}
\newcommand{\Vlambda}    {\boldsymbol{\uplambda}}
\newcommand{\Vmu}        {\boldsymbol{\upmu}}
\newcommand{\Vnu}        {\boldsymbol{\upnu}}
\newcommand{\Vxi}        {\boldsymbol{\upxi}}
\newcommand{\Vpi}        {\boldsymbol{\uppi}}
\newcommand{\Vvarpi}     {\boldsymbol{\upvarpi}}
\newcommand{\Vrho}       {\boldsymbol{\uprho}}
\newcommand{\Vvarrho}    {\boldsymbol{\upvarrho}}
\newcommand{\Vsigma}     {\boldsymbol{\upsigma}}
\newcommand{\Vvarsigma}  {\boldsymbol{\upvarsigma}}
\newcommand{\Vtau}       {\boldsymbol{\uptau}}
\newcommand{\Vupsilon}   {\boldsymbol{\upupsilon}}
\newcommand{\Vphi}       {\boldsymbol{\upphi}}
\newcommand{\Vvarphi}    {\boldsymbol{\upvarphi}}
\newcommand{\Vchi}       {\boldsymbol{\upchi}}
\newcommand{\Vpsi}       {\boldsymbol{\uppsi}}
\newcommand{\Vomega}     {\boldsymbol{\upomega}}

% _B_old italicised lower case Greek letters
\newcommand{\Balpha}     {\boldsymbol{\alpha}}
\newcommand{\Bbeta}      {\boldsymbol{\beta}}
\newcommand{\Bgamma}     {\boldsymbol{\gamma}}
\newcommand{\Bdelta}     {\boldsymbol{\delta}}
\newcommand{\Bepsilon}   {\boldsymbol{\epsilon}}
\newcommand{\Bvarepsilon}{\boldsymbol{\varepsilon}}
\newcommand{\Bzeta}      {\boldsymbol{\zeta}}
\newcommand{\Beta}       {\boldsymbol{\eta}}                % \Beta=B undefined
\newcommand{\Btheta}     {\boldsymbol{\theta}}
\newcommand{\Bvartheta}  {\boldsymbol{\vartheta}}
\newcommand{\Biota}      {\boldsymbol{\iota}}
\newcommand{\Bkappa}     {\boldsymbol{\kappa}}
\newcommand{\Blambda}    {\boldsymbol{\lambda}}
\newcommand{\Bmu}        {\boldsymbol{\mu}}
\newcommand{\Bnu}        {\boldsymbol{\nu}}
\newcommand{\Bxi}        {\boldsymbol{\xi}}
\newcommand{\Bpi}        {\boldsymbol{\pi}}
\newcommand{\Bvarpi}     {\boldsymbol{\varpi}}
\newcommand{\Brho}       {\boldsymbol{\rho}}
\newcommand{\Bvarrho}    {\boldsymbol{\varrho}}
\newcommand{\Bsigma}     {\boldsymbol{\sigma}}
\newcommand{\Bvarsigma}  {\boldsymbol{\varsigma}}
\newcommand{\Btau}       {\boldsymbol{\tau}}
\newcommand{\Bupsilon}   {\boldsymbol{\upsilon}}
\newcommand{\Bphi}       {\boldsymbol{\phi}}
\newcommand{\Bvarphi}    {\boldsymbol{\phi}}
\newcommand{\Bchi}       {\boldsymbol{\chi}}
\newcommand{\Bpsi}       {\boldsymbol{\psi}}
\newcommand{\Bomega}     {\boldsymbol{\omega}}

% Roman capital letters (for matrices)

\newcommand{\Amat}{{\rm A}}
\newcommand{\Bmat}{{\rm B}}
\newcommand{\Cmat}{{\rm C}}
\newcommand{\Dmat}{{\rm D}}
\newcommand{\Emat}{{\rm E}}
\newcommand{\Fmat}{{\rm F}}
\newcommand{\Gmat}{{\rm G}}
\newcommand{\Hmat}{{\rm H}}
\newcommand{\Imat}{{\rm I}}
\newcommand{\Jmat}{{\rm J}}
\newcommand{\Kmat}{{\rm K}}
\newcommand{\Lmat}{{\rm L}}
\newcommand{\Mmat}{{\rm M}}
\newcommand{\Nmat}{{\rm N}}
\newcommand{\Omat}{{\rm O}}
\newcommand{\Pmat}{{\rm P}}
\newcommand{\Qmat}{{\rm Q}}
\newcommand{\Rmat}{{\rm R}}
\newcommand{\Smat}{{\rm S}}
\newcommand{\Tmat}{{\rm T}}
\newcommand{\Umat}{{\rm U}}
\newcommand{\Vmat}{{\rm V}}
\newcommand{\Wmat}{{\rm W}}
\newcommand{\Xmat}{{\rm X}}
\newcommand{\Ymat}{{\rm Y}}
\newcommand{\Zmat}{{\rm Z}}

% Sans serif letters in math mode

\newcommand{\Asf}{\mathsf{A}}
\newcommand{\Bsf}{\mathsf{B}}
\newcommand{\Csf}{\mathsf{C}}
\newcommand{\Dsf}{\mathsf{D}}
\newcommand{\Esf}{\mathsf{E}}
\newcommand{\Fsf}{\mathsf{F}}
\newcommand{\Gsf}{\mathsf{G}}
\newcommand{\Hsf}{\mathsf{H}}
\newcommand{\Isf}{\mathsf{I}}
\newcommand{\Jsf}{\mathsf{J}}
\newcommand{\Ksf}{\mathsf{K}}
\newcommand{\Lsf}{\mathsf{L}}
\newcommand{\Msf}{\mathsf{M}}
\newcommand{\Nsf}{\mathsf{N}}
\newcommand{\Osf}{\mathsf{O}}
\newcommand{\Psf}{\mathsf{P}}
\newcommand{\Qsf}{\mathsf{Q}}
\newcommand{\Rsf}{\mathsf{R}}
\newcommand{\Ssf}{\mathsf{S}}
\newcommand{\Tsf}{\mathsf{T}}
\newcommand{\Usf}{\mathsf{U}}
\newcommand{\Vsf}{\mathsf{V}}
\newcommand{\Wsf}{\mathsf{W}}
\newcommand{\Xsf}{\mathsf{X}}
\newcommand{\Ysf}{\mathsf{Y}}
\newcommand{\Zsf}{\mathsf{Z}}

% Calligraphic characters
% Comment Axel Obermeier: inconsistent - why not \CA etc. for upper case?
%                         Added below for usage in exercise, so that everything is collected in one place
%                         Redundant until this is replaced

\providecommand{\Ca}{{\cal A}}
\providecommand{\Cb}{{\cal B}}
\providecommand{\Cc}{{\cal C}}
\providecommand{\Cd}{{\cal D}}
\providecommand{\Ce}{{\cal E}}
\providecommand{\Cf}{{\cal F}}
\providecommand{\Cg}{{\cal G}}
\providecommand{\Ch}{{\cal H}}
\providecommand{\Ci}{{\cal I}}
\providecommand{\Cj}{{\cal J}}
\providecommand{\Ck}{{\cal K}}
\providecommand{\Cl}{{\cal L}}
\providecommand{\Cm}{{\cal M}}
\providecommand{\Cn}{{\cal N}}
\providecommand{\Co}{{\cal O}}
\providecommand{\Cp}{{\cal P}}
\providecommand{\Cq}{{\cal Q}}
\providecommand{\Cr}{{\cal R}}
\providecommand{\Cs}{{\cal S}}
\providecommand{\Ct}{{\cal T}}
\providecommand{\Cu}{{\cal U}}
\providecommand{\Cv}{{\cal V}}
\providecommand{\Cw}{{\cal W}}
\providecommand{\Cx}{{\cal X}}
\providecommand{\Cy}{{\cal Y}}
\providecommand{\Cz}{{\cal Z}}

\providecommand{\CA}{{\cal A}}
\providecommand{\CB}{{\cal B}}
\providecommand{\CC}{{\cal C}}
\providecommand{\CD}{{\cal D}}
\providecommand{\CE}{{\cal E}}
\providecommand{\CF}{{\cal F}}
\providecommand{\CG}{{\cal G}}
\providecommand{\CH}{{\cal H}}
\providecommand{\CI}{{\cal I}}
\providecommand{\CJ}{{\cal J}}
\providecommand{\CK}{{\cal K}}
\providecommand{\CL}{{\cal L}}
\providecommand{\CM}{{\cal M}}
\providecommand{\CN}{{\cal N}}
\providecommand{\CO}{{\cal O}}
\providecommand{\CP}{{\cal P}}
\providecommand{\CQ}{{\cal Q}}
\providecommand{\CR}{{\cal R}}
\providecommand{\CS}{{\cal S}}
\providecommand{\CT}{{\cal T}}
\providecommand{\CU}{{\cal U}}
\providecommand{\CV}{{\cal V}}
\providecommand{\CW}{{\cal W}}
\providecommand{\CX}{{\cal X}}
\providecommand{\CY}{{\cal Y}}
\providecommand{\CZ}{{\cal Z}}

% Calligraphic characters bold

\newcommand{\Cav}{\boldsymbol {\cal A}}
\newcommand{\Cbv}{\boldsymbol {\cal B}}
\newcommand{\Ccv}{\boldsymbol {\cal C}}
\newcommand{\Cdv}{\boldsymbol {\cal D}}
\newcommand{\Cev}{\boldsymbol {\cal E}}
\newcommand{\Cfv}{\boldsymbol {\cal F}}
\newcommand{\Cgv}{\boldsymbol {\cal G}}
\newcommand{\Chv}{\boldsymbol {\cal H}}
\newcommand{\Civ}{\boldsymbol {\cal I}}
\newcommand{\Cjv}{\boldsymbol {\cal J}}
\newcommand{\Ckv}{\boldsymbol {\cal K}}
\newcommand{\Clv}{\boldsymbol {\cal L}}
\newcommand{\Cmv}{\boldsymbol {\cal M}}
\newcommand{\Cnv}{\boldsymbol {\cal N}}
\newcommand{\Cov}{\boldsymbol {\cal O}}
\newcommand{\Cpv}{\boldsymbol {\cal P}}
\newcommand{\Cqv}{\boldsymbol {\cal Q}}
\newcommand{\Crv}{\boldsymbol {\cal R}}
\newcommand{\Csv}{\boldsymbol {\cal S}}
\newcommand{\Ctv}{\boldsymbol {\cal T}}
\newcommand{\Cuv}{\boldsymbol {\cal U}}
\newcommand{\Cvv}{\boldsymbol {\cal V}}
\newcommand{\Cwv}{\boldsymbol {\cal W}}
\newcommand{\Cxv}{\boldsymbol {\cal X}}
\newcommand{\Cyv}{\boldsymbol {\cal Y}}
\newcommand{\Czv}{\boldsymbol {\cal Z}}

% Blackboard bold characters

\providecommand{\bbA}{\mathbb{A}}
\providecommand{\bbB}{\mathbb{B}}
\providecommand{\bbC}{\mathbb{C}}
\providecommand{\bbD}{\mathbb{D}}
\providecommand{\bbE}{\mathbb{E}}
\providecommand{\bbF}{\mathbb{F}}
\providecommand{\bbG}{\mathbb{G}}
\providecommand{\bbH}{\mathbb{H}}
\providecommand{\bbI}{\mathbb{I}}
\providecommand{\bbJ}{\mathbb{J}}
\providecommand{\bbK}{\mathbb{K}}
\providecommand{\bbL}{\mathbb{L}}
\providecommand{\bbM}{\mathbb{M}}
\providecommand{\bbN}{\mathbb{N}}
\providecommand{\bbO}{\mathbb{O}}
\providecommand{\bbP}{\mathbb{P}}
\providecommand{\bbQ}{\mathbb{Q}}
\providecommand{\bbR}{\mathbb{R}}
\providecommand{\bbS}{\mathbb{S}}
\providecommand{\bbT}{\mathbb{T}}
\providecommand{\bbU}{\mathbb{U}}
\providecommand{\bbV}{\mathbb{V}}
\providecommand{\bbW}{\mathbb{W}}
\providecommand{\bbX}{\mathbb{X}}
\providecommand{\bbY}{\mathbb{Y}}
\providecommand{\bbZ}{\mathbb{Z}}

% Special boldface characters
\providecommand{\reel}{\bbR}
\newcommand{\nat}{\bbN}
\newcommand{\ganz}{\bbZ}
\providecommand{\comp}{\bbC}

% Euler font ("Fraktur"))

\providecommand{\FA}{\mathfrak{A}}
\providecommand{\FB}{\mathfrak{B}}
\providecommand{\FC}{\mathfrak{C}}
\providecommand{\FD}{\mathfrak{D}}
\providecommand{\FE}{\mathfrak{E}}
\providecommand{\FF}{\mathfrak{F}}
\providecommand{\FG}{\mathfrak{G}}
\providecommand{\FH}{\mathfrak{H}}
\providecommand{\FI}{\mathfrak{I}}
\providecommand{\FJ}{\mathfrak{J}}
\providecommand{\FK}{\mathfrak{K}}
\providecommand{\FL}{\mathfrak{L}}
\providecommand{\FM}{\mathfrak{M}}
\providecommand{\FN}{\mathfrak{N}}
\providecommand{\FO}{\mathfrak{O}}
\providecommand{\FP}{\mathfrak{P}}
\providecommand{\FQ}{\mathfrak{Q}}
\providecommand{\FR}{\mathfrak{R}}
\providecommand{\FS}{\mathfrak{S}}
\providecommand{\FT}{\mathfrak{T}}
\providecommand{\FU}{\mathfrak{U}}
\providecommand{\FV}{\mathfrak{V}}
\providecommand{\FW}{\mathfrak{W}}
\providecommand{\FX}{\mathfrak{X}}
\providecommand{\FY}{\mathfrak{Y}}
\providecommand{\FZ}{\mathfrak{Z}}

\providecommand{\Fa}{\mathfrak{a}}
\providecommand{\Fb}{\mathfrak{b}}
\providecommand{\Fc}{\mathfrak{c}}
\providecommand{\Fd}{\mathfrak{d}}
\providecommand{\Fe}{\mathfrak{e}}
\providecommand{\Ff}{\mathfrak{f}}
\providecommand{\Fg}{\mathfrak{g}}
\providecommand{\Fh}{\mathfrak{h}}
\providecommand{\Fi}{\mathfrak{i}}
\providecommand{\Fj}{\mathfrak{j}}
\providecommand{\Fk}{\mathfrak{k}}
\providecommand{\Fl}{\mathfrak{l}}
\providecommand{\Fm}{\mathfrak{m}}
\providecommand{\Fn}{\mathfrak{n}}
\providecommand{\Fo}{\mathfrak{o}}
\providecommand{\Fp}{\mathfrak{p}}
\providecommand{\Fq}{\mathfrak{q}}
\providecommand{\Fr}{\mathfrak{r}}
\providecommand{\Fs}{\mathfrak{s}}
\providecommand{\Ft}{\mathfrak{t}}
\providecommand{\Fu}{\mathfrak{u}}
\providecommand{\Fv}{\mathfrak{v}}
\providecommand{\Fw}{\mathfrak{w}}
\providecommand{\Fx}{\mathfrak{x}}
\providecommand{\Fy}{\mathfrak{y}}
\providecommand{\Fz}{\mathfrak{z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros for convenience
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\EUSP}[2]{\left<{#1},{#2}\right>} % Euclidean inner product
\newcommand*{\DP}[2]{\left<{#1},{#2}\right>} % Duality product
\newcommand*{\cross}[2]{{#1}\times{#2}}       %Cross product of vectors in R^3

\providecommand*{\wt}[1]{\widetilde{#1}}
\providecommand*{\wh}[1]{\widehat{#1}}
\providecommand{\DS}{\displaystyle}
\newcommand{\dis}{\displaystyle}

% Abstract Norms and inner producrs

\providecommand*{\N}[1]{\left\|{#1}\right\|} % Double bar norm
\newcommand*{\IP}[2]{\left({#1},{#2}\right)} % Bracket inner product, same as \SP
\providecommand*{\NN}[1]{\N{#1}_{0}}         % Zero norm
\newcommand*{\SN}[1]{\left|{#1}\right|}      % Single bar norm
\providecommand*{\abs}[1]{\left|{#1}\right|} % absolute value, same as \SN
\newcommand*{\SP}[2]{\left({#1},{#2}\right)} % Inner product
\newcommand{\xLinf}[1]{L^{\infty}({#1})}
\newcommand{\NxLinf}[2]{\left\|{#1}\right\|_{\xLinf{#2}}}
\newcommand*{\NxLone}[2]{\left\|{#1}\right\|_{L^{1}({#2})}}
\newcommand*{\NxLtwo}[2]{\left\|{#1}\right\|_{L^{2}({#2})}}
\newcommand*{\Pol}[1]{\Cp_{#1}}
\newcommand*{\Spline}[2]{\Cs_{#1,#2}}

% Lebesgue measure
\newcommand{\DX}{\mathrm{d}\Bx}
\newcommand{\dS}{\mathrm{d}S}
\providecommand{\ds}{\mathrm{d}\vec{\Bs}}

% Embeddings
\newcommand{\compemb}{\overset{c}{\hookrightarrow}} % compact embedding
\newcommand{\contemb}{\hookrightarrow}              % continuous embedding

% Modifiers

\newcommand*{\mat}[1]{\mathbf{#1}} % matrices
\newcommand*{\Op}[1]{\mathsf{#1}} % Operators
\newcommand*{\blf}[1]{\mathsf{#1}} % Bilinear forms
\newcommand*{\cvec}[1]{\vec{#1}} % Coefficient vector
\newcommand*{\conj}[1]{\overline{#1}} % complex conjugate

% restriction
\newcommand*{\rst}[2]{\left.\mathstrut#1\right|_{#2}}

% Default domains and boundaries (can be adjusted !)
\newcommand{\defaultdomain}{\Omega}
\newcommand{\defaultboundary}{\partial\defaultdomain}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SPACES and NORMS
% First argument (optional) domain
%                (-> default = \defaultdomain, \defaultboundary)
% Second argument for norms \Nxxx, \SNxxx gives the function
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% L^p spaces

\providecommand*{\Lp}[2][\defaultdomain]{L^{#2}({#1})}
\newcommand*{\Lpv}[2][\defaultdomain]{\BL^{#2}({#1})}
\newcommand*{\NLp}[3][\defaultdomain]{\N{#2}_{\Lp[#1]{#3}}}
\newcommand*{\NLpv}[3][\defaultdomain]{\N{#2}_{\Lpv[#1]{#3}}}

% Special L^p spaces
\newcommand*{\Ltwo}[1][\defaultdomain]{\Lp[#1]{2}}
\newcommand*{\Ltwov}[1][\defaultdomain]{\Lpv[#1]{2}}
\newcommand*{\NLtwo}[2][\defaultdomain]{\NLp[#1]{#2}{2}}
\newcommand*{\NLtwov}[2][\defaultdomain]{\NLpv[#1]{#2}{2}}
\newcommand*{\SPLtwo}[3][\defaultdomain]{\SP{#2}{#3}_{\Ltwo[#1]}}
\newcommand*{\Linf}[1][\defaultdomain]{L^{\infty}({#1})}
\newcommand*{\NLinf}[2][\defaultdomain]{\N{#2}_{\Linf[{#1}]}}

% little l^p spaces (for sequencies)
\newcommand{\defaultseqdomain}{\bbZ}
\newcommand*{\lp}[2][\defaultseqdomain]{l^{#2}({#1})}
\newcommand*{\lpv}[2][\defaultseqdomain]{\Bl^{#2}({#1})}
\newcommand*{\Nlp}[3][\defaultseqdomain]{\N{#2}_{\lp[#1]{#3}}}
\newcommand*{\Nlpv}[3][\defaultseqdomain]{\N{#2}_{\lpv[#1]{#3}}}
\newcommand*{\ltwo}[1][\defaultseqdomain]{\lp[#1]{2}}
\newcommand*{\ltwov}[1][\defaultseqdomain]{\lpv[#1]{2}}
\newcommand*{\Nltwo}[2][\defaultseqdomain]{\Nlp[#1]{#2}{2}}
\newcommand*{\Nltwov}[2][\defaultseqdomain]{\Nlpv[#1]{#2}{2}}
\newcommand*{\linf}[1][\defaultseqdomain]{l^{\infty}({#1})}
\newcommand*{\Nlinf}[2][\defaultseqdomain]{\N{#2}_{\linf[{#1}]}}

% Sobolev spaces for general L^p spaces
% first argument (optional) = domain,
% second argument: differentiation order
% third argument: underlying L^p space
% (for norms the second argument provides the function)
\newcommand*{\Wmp}[3][\defaultdomain]{W^{{#2},{#3}}({#1})}
\newcommand*{\Wmpv}[3][\defaultdomain]{\BW^{{#2},{#3}}({#1})}
\newcommand*{\bWmp}[4][\defaultdomain]{W_{#4}^{{#2},{#3}}({#1})}    % boundary values
\newcommand*{\bWmpv}[4][\defaultdomain]{\BW_{#4}^{{#2},{#3}}({#1})}
\newcommand*{\zbWmp}[3][\defaultdomain]{\bWmp[#1]{#2}{#3}{0}}       % zero b.v.
\newcommand*{\zbWmpv}[3][\defaultdomain]{\bWmpv[#1]{#2}{#3}{0}}
\newcommand*{\NWmp}[4][\defaultdomain]{\N{#2}_{\Wmp[#1]{#3}{#4}}}
\newcommand*{\NWmpv}[4][\defaultdomain]{\N{#2}_{\Wmpv[#1]{#3}{#4}}}
\newcommand*{\SNWmp}[4][\defaultdomain]{\SN{#2}_{\Wmp[#1]{#3}{#4}}}
\newcommand*{\SNWmpv}[4][\defaultdomain]{\SN{#2}_{\Wmp[#1]{#3}{#4}}}

% Sobolev spaces for p=2
\newcommand*{\Hm}[2][\defaultdomain]{H^{#2}({#1})}
\newcommand*{\Hmv}[2][\defaultdomain]{\BH^{#2}({#1})}
\newcommand*{\bHm}[3][\defaultdomain]{H_{#3}^{#2}({#1})}
\newcommand*{\zbHm}[3][\defaultdomain]{\bHm[#1]{#2}{0}}
\newcommand*{\bHmv}[3][\defaultdomain]{\BH_{#3}^{#2}({#1})}
\newcommand*{\zbHmv}[3][\defaultdomain]{\bHmv[#1]{#2}{0}}
\newcommand*{\NHm}[3][\defaultdomain]{{\N{#2}}_{\Hm[{#1}]{#3}}}
\newcommand*{\NHmv}[3][\defaultdomain]{{\N{#2}}_{\Hmv[{#1}]{#3}}}
\newcommand*{\SNHm}[3][\defaultdomain]{{\SN{#2}}_{\Hm[{#1}]{#3}}}
\newcommand*{\SNHmv}[3][\defaultdomain]{{\SN{#2}}_{\Hmv[{#1}]{#3}}}

% Special Sobolev spaces for p=2
\newcommand*{\Hone}[1][\defaultdomain]{\Hm[#1]{1}}
\newcommand*{\Honev}[1][\defaultdomain]{\Hmv[#1]{1}}
\newcommand*{\bHone}[2][\defaultdomain]{\bHm[#1]{1}{#2}}
\newcommand*{\bHonev}[2][\defaultdomain]{\bHmv[#1]{1}{#2}}
\newcommand*{\zbHone}[1][\defaultdomain]{\bHm[#1]{1}{0}}
\newcommand*{\zbHonev}[1][\defaultdomain]{\bHmv[#1]{1}{0}}
\newcommand*{\NHone}[2][\defaultdomain]{{\N{#2}}_{\Hone[{#1}]}}
\newcommand*{\NHonev}[2][\defaultdomain]{{\N{#2}}_{\Honev[{#1}]}}
\newcommand*{\SNHone}[2][\defaultdomain]{{\SN{#2}}_{\Hone[{#1}]}}
\newcommand*{\SNHonev}[2][\defaultdomain]{{\SN{#2}}_{\Honev[{#1}]}}

\newcommand{\hlb}{\frac{1}{2}}
\providecommand*{\Hh}[1][\defaultboundary]{\Hm[#1]{\hlb}}
\newcommand*{\Hhv}[1][\defaultboundary]{\Hmv[#1]{\hlb}}
\newcommand*{\NHh}[2][\defaultboundary]{\N{#2}_{\Hh[#1]}}
\newcommand*{\NHhv}[2][\defaultboundary]{\N{#2}_{\Hhv[#1]}}
\newcommand*{\SNHh}[2][\defaultboundary]{\SN{#2}_{\Hh[#1]}}
\newcommand*{\SNHhv}[2][\defaultboundary]{\SN{#2}_{\Hhv[#1]}}

% Hdiv
\newcommand*{\Hdiv}[1][\defaultdomain]{\boldsymbol{H}(\Div,{#1})}
\newcommand*{\bHdiv}[2][\defaultdomain]{\boldsymbol{H}_{#2}(\Div,{#1})}
\newcommand*{\zbHdiv}[1][\defaultdomain]{\bHdiv[#1]{0}}
\newcommand*{\kHdiv}[1][\defaultdomain]{\boldsymbol{H}(\Div0,{#1})}
\newcommand*{\bkHdiv}[2][\defaultdomain]{\boldsymbol{H}_{#2}(\Div0,{#1})}
\newcommand*{\zbkHdiv}[1][\defaultdomain]{\bkHdiv[#1]{0}}
\newcommand*{\NHdiv}[2][\defaultdomain]{\N{#2}_{\Hdiv[#1]}}
\newcommand{\Honediv}[1][\defaultdomain]{\boldsymbol{H}^{1}_{0}(\Div0,{#1})} 

% Hcurl
\newcommand*{\Hcurl}[1][\defaultdomain]{\boldsymbol{H}(\curl,{#1})}
\newcommand*{\bHcurl}[2][\defaultdomain]{\boldsymbol{H}_{#2}(\curl,{#1})}
\newcommand*{\zbHcurl}[1][\defaultdomain]{\bHcurl[#1]{0}}
\newcommand*{\kHcurl}[1][\defaultdomain]{\boldsymbol{H}(\curl0,{#1})}
\newcommand*{\bkHcurl}[2][\defaultdomain]{\boldsymbol{H}_{#2}(\curl0,{#1})}
\newcommand*{\zbkHcurl}[1][\defaultdomain]{\bkHcurl[#1]{0}}
\newcommand*{\NHcurl}[2][\defaultdomain]{\N{#2}_{\Hcurl[#1]}}

% Spaces of continuously differentiable functions
\newcommand*{\Contm}[2][\defaultdomain]{C^{#2}({#1})}
\newcommand*{\Contmv}[2][\defaultdomain]{\BC^{#2}({#1})}
\newcommand*{\NContm}[3][\defaultdomain]{\N{#2}_{\Cm[#1]{#3}}}
\newcommand*{\NContmv}[3][\defaultdomain]{\N{#2}_{\Cmv[#1]{#3}}}

% Bochner spaces for evolution problems
\newcommand{\period}{]0,T[}
\newcommand{\cperiod}{]0,T[}
\newcommand*{\TLtwo}[2][\period]{L^2({#1};{#2})}
\newcommand*{\TLinf}[2][\period]{L^{\infty}({#1};{#2})}
\newcommand*{\TCont}[2][\cperiod]{C^{0}({#1};{#2})}
\newcommand*{\THm}[3][\period]{H^{#2}({#1};{#3})}

% Functions of bounded variation
\newcommand*{\BdV}[1][\defaultdomain]{BV_{\mathrm{loc}}({#1})}

% Jumps and averages

\newcommand*{\jump}[2][]{\left[{#2}\right]_{#1}}
\newcommand*{\avg}[2][]{\left\{{#2}\right\}_{#1}}

% partial derivatives
\newcommand*{\Dp}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand*{\DDp}[2]{\frac{\partial^2{#1}}{\partial{#2}^2}}
\newcommand*{\DpDp}[3]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}}
\newcommand*{\dtemp}[1]{\frac{\partial {#1}}{\partial t}}
\newcommand*{\ddtemp}[1]{\frac{\partial^2 {#1}}{\partial t^2}}

% intervals
\newcommand{\ointv}[1]{]{#1}[}
\newcommand{\cintv}[1]{[{#1}]}
\newcommand{\ocintv}[1]{]{#1}]}
\newcommand{\cointv}[1]{[{#1}[}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

